Feasibility of assessing cognitive impairment via distributed camera network and privacy-preserving edge computing

INTRODUCTION: Mild cognitive impairment (MCI) is characterized by a decline in cognitive functions beyond typical age and education-related expectations. Since, MCI has been linked to reduced social interactions and increased aimless movements, we aimed to automate the capture of these behaviors to enhance longitudinal monitoring. METHODS: Using a privacy-preserving distributed camera network, we collected movement and social interaction data from groups of individuals with MCI undergoing therapy within a 1700$m^2$ space. We developed movement and social interaction features, which were then used to train a series of machine learning algorithms to distinguish between higher and lower cognitive functioning MCI groups. RESULTS: A Wilcoxon rank-sum test revealed statistically significant differences between high and low-functioning cohorts in features such as linear path length, walking speed, change in direction while walking, entropy of velocity and direction change, and number of group formations in the indoor space. Despite lacking individual identifiers to associate with specific levels of MCI, a machine learning approach using the most significant features provided a 71% accuracy. DISCUSSION: We provide evidence to show that a privacy-preserving low-cost camera network using edge computing framework has the potential to distinguish between different levels of cognitive impairment from the movements and social interactions captured during group activities.

==> tables/results.tex <==
\begin{table*}[t]
    \centering
    \caption{Precision, recall, F1 score and accuracy along with 95\% confidence intervals when SVM, XGBoost, logistic regression and lasso binary classifications were used with all the features, only social interaction features and only movement features.
    (\textbf{Bold} shows the best performance.)}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        \textbf{Metrics} & \multicolumn{4}{|c|}{\textbf{All features}} & \multicolumn{4}{|c|}{\textbf{Social interaction features}} & \multicolumn{4}{|c|}{\textbf{Movement features}} \\
        \hline
         & SVM & XGB & LR & Lasso & SVM & XGB & LR & Lasso & SVM & XGB & LR & Lasso \\
         \hline
       Precision & $0.62\pm0.054$ & \textbf{0.69$\pm$0.051} & $0.65\pm0.053$ & $0.67\pm0.052$ & $0.63\pm0.053$ & $0.64\pm0.053$ & $0.62\pm0.054$ & $0.63\pm0.053$ & $0.64\pm0.053$ & $0.64\pm0.053$ & $0.65\pm0.053$ & $0.66\pm0.052$\\
        \hline
        Recall & \textbf{0.72$\pm$0.050} & $0.66\pm0.052$ & $0.65\pm0.053$ & $0.64\pm0.053$ & $0.71\pm0.050$ & $0.64\pm0.053$ & $0.62\pm0.054$ & $0.63\pm0.053$ & $0.70\pm0.051$ & $0.59\pm0.054$ & $0.57\pm0.055$ & $0.59\pm0.054$\\
        \hline
        F1 score & $0.67\pm0.052$ & \textbf{0.68$\pm$0.052} & $0.65\pm0.053$ & $0.65\pm0.053$ & $0.67\pm0.052$ & $0.64\pm0.053$ & $0.62\pm0.054$ & $0.63\pm0.053$ & $0.67\pm0.052$ & $0.61\pm0.054$ & $0.60\pm0.054$ & $0.62\pm0.054$\\
        \hline
        Accuracy & $0.66\pm0.052$ & \textbf{0.71$\pm$0.050} & $0.68\pm0.052$ & $0.68\pm0.051$ & $0.67\pm0.052$ & $0.67\pm0.052$ & $0.64\pm0.053$ & $0.66\pm0.052$ & $0.68\pm0.052$ & $0.65\pm0.053$ & $0.65\pm0.053$ & $0.66\pm0.052$\\
        \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:moca_classification}
\end{table*}
